Wave Chaos in Quantum Pseudointegrable Billiards

We clarify from a general perspective, the condition for the appearance of chaotic energy spectrum in quantum pseudointegrable billiards with a point scatterer inside.

==> ps_inc.tex <==
\sbox{\plotpoint}{\rule[-0.200pt]{1.000pt}{1.000pt}}%


